From Logistic Regression to the Perceptron Algorithm: Exploring Gradient Descent with Large Step Sizes

We focus on the classification problem with a separable dataset, one of the most important and classical problems from machine learning. The standard approach to this task is logistic regression with gradient descent (LR+GD). Recent studies have observed that LR+GD can find a solution with arbitrarily large step sizes, defying conventional optimization theory. Our work investigates this phenomenon and makes three interconnected key observations about LR+GD with large step sizes. First, we find a remarkably simple explanation of why LR+GD with large step sizes solves the classification problem: LR+GD reduces to a batch version of the celebrated perceptron algorithm when the step size $\gamma \to \infty.$ Second, we observe that larger step sizes lead LR+GD to higher logistic losses when it tends to the perceptron algorithm, but larger step sizes also lead to faster convergence to a solution for the classification problem, meaning that logistic loss is an unreliable metric of the proximity to a solution. Surprisingly, high loss values can actually indicate faster convergence. Third, since the convergence rate in terms of loss function values of LR+GD is unreliable, we examine the iteration complexity required by LR+GD with large step sizes to solve the classification problem and prove that this complexity is suboptimal. To address this, we propose a new method, Normalized LR+GD - based on the connection between LR+GD and the perceptron algorithm - with much better theoretical guarantees.

==> results_2024/plot_local_optimization_2024_paper_new_algorithm_0_table.tex <==
\begin{tabular}{|c|c|}
{Method} & {\# of Iterations} \\
Normalized LR+GD Step: 100.0 & \textbf{7647} \\
Normalized LR+GD Step: 10.0 & 7664 \\
Normalized LR+GD Step: 1.0 & 7674 \\
LR+GD Step: 10.0 & 8862 \\
Normalized LR+GD Step: 0.1 & 9379 \\
\end{tabular}

==> results_2024/plot_local_optimization_2024_paper_new_algorithm_4_table.tex <==
\begin{tabular}{|c|c|}
{Method} & {\# of Iterations} \\
LR+GD Step: 10.0 & \textbf{142652} \\
LR+GD Step: 100.0 & 143314 \\
LR+GD Step: 1.0 & 166384 \\
Normalized LR+GD Step: 10.0 & 197525 \\
Normalized LR+GD Step: 100.0 & 199367 \\
\end{tabular}

==> results_2024/tmp.tex <==
\begin{table}[H]
\centering
\caption{# of iterations to find a solution. \label{tbl:acc}}
\begin{tabular}{|c|c|}
{Method} & {# of Iterations} \\
LR+GD Step: 10.0 & \textbf{2778} \\
LR+GD Step: 100.0 & 2928 \\
Normalized LR+GD Step: 100.0 & 3160 \\
Normalized LR+GD Step: 1.0 & 3351 \\
Normalized LR+GD Step: 10.0 & 3359 \\
Normalized LR+GD Step: 0.1 & 5816 \\
Normalized LR+GD Step: 0.01 & 20407 \\
LR+GD Step: 1.0 & 21012 \\
Normalized LR+GD Step: 0.001 & 204082 \\
LR+GD Step: 0.1 & 210089 \\
LR+GD Step: 0.001 & nan \\
LR+GD Step: 0.01 & nan \\
\end{tabular}
\end{table}

